A Solution to Adaptive Mobile Manipulator Throwing

Mobile manipulator throwing is a promising method to increase the flexibility and efficiency of dynamic manipulation in factories. Its major challenge is to efficiently plan a feasible throw under a wide set of task specifications. We show that the mobile manipulator throwing problem can be simplified to a planar problem, hence greatly reducing the computational costs. Using machine learning approaches, we build a model of the object's inverted flying dynamics and the robot's kinematic feasibility, which enables throwing motion generation within 1 ms for given query of target position. Thanks to the computational efficiency of our method, we show that the system is adaptive under disturbance, via replanning on the fly for alternative solutions, instead of sticking to the original throwing plan.

==> sections/backup.tex <==
\begin{algorithm}
  \SetAlgoLined
  \caption{Algorithm to get velocity hedgehog}
  \Input{robot model with forward kinematics and differential forward kinematics $robot$}
  \Output{max\_z\_phi\_gamma, q\_z\_phi\_gamma}
  \Data{robot joint position limit $(q_{min}, q_{max})$,\\ 
        robot joint velocity limit $\dot{q}_{max}$,\\
        joint grid size $\Delta q$, \\ 
        velocity hedgehog grids $Z, \Phi, \Gamma$\linebreak}%\Delta z, \Delta \phi, \Delta \gamma$}
  
  % \nosemic
  % \dosemic\nonl \textbf{Build robot dataset $\mathcal{X}$}\\
  \tcc{Build robot dataset $\mathcal{X}$}
 % $M \gets ComputeSize(q_{min}, q_{max}, \Delta q)$ 
  $\mathcal{Q}  \gets ComputeMesh(q_{min}, q_{max}, \Delta q)$ \\
  $\mathcal{X} \gets empty$ \\
  \For {$i = 1$ to $\#\mathcal{Q}$} {
  $q \gets \mathcal{Q}_i$ \\
  $x, y, z \gets robot.fkine(q).translation$ \\
  \tcc{Filter out robot configuration that is not stretched}
  \If {$Norm(x,y) < stretch\_thres$}{
    continue}

  $J \gets robot.jacob(q)$ \\
  $u, s, vh \gets SVD(J)$ \\
  \tcc{Filter out robot configuration with low manipulability index}
  \If {$Min(s) < singular\_thres$}{
    continue}
  $data \gets (q, z, J)$ \\
  $\mathcal{X}.add(data)$ \\
}
% \dosemic\nonl \textbf{Group data by $Z$}\\
\tcc{Group data by $Z$}
$\{\mathcal{X}_z\} \gets GroupBy(\mathcal{X}, Z)$\\
% \dosemic\nonl \textbf{Initialize velocity hedgehog}\\
\tcc{Initialize velocity hedgehog}
$\text{max\_z\_phi\_gamma} \gets zeros([\#Z, \#\Phi, \#\Gamma])$\\
$\text{q\_z\_phi\_gamma} \gets arrays([\#Z, \#\Phi, \#\Gamma, \#joints])$\\
% \dosemic\nonl \textbf{Build velocity hedgehog}\\
\tcc{Build velocity hedgehog}
\For{$z \in Z$}{
    \For{$\phi \in \Phi$}{
        \For{$\gamma \in \Gamma$}{
            \For{$data \in \mathcal{X}_z$}{
                \tcc{Get max. speed along ($\phi, \gamma$) at joint configuration $q$ under joint velocity limit $\dot{q}_{max}$}
                $res \gets LP(\phi, \gamma, data.q, robot, \dot{q}_{max})$\\
                \If {$res > \text{max\_z\_phi\_gamma}(z, \phi, \gamma)$}{
                    $\text{max\_z\_phi\_gamma}(z, \phi, \gamma) \gets res$\\
                    $\text{q\_z\_phi\_gamma}(z, \phi, \gamma) \gets data.q$
                }
            }
        }
    }
}
\Return $\text{max\_z\_phi\_gamma}, \text{q\_z\_phi\_gamma}$
\label{algo:hedgehog}
\end{algorithm}
